OCRTurk: A Comprehensive OCR Benchmark for Turkish

Document parsing is now widely used in applications, such as large-scale document digitization, retrieval-augmented generation, and domain-specific pipelines in healthcare and education. Benchmarking these models is crucial for assessing their reliability and practical robustness. Existing benchmarks mostly target high-resource languages and provide limited coverage for low-resource settings, such as Turkish. Moreover, existing studies on Turkish document parsing lack a standardized benchmark that reflects real-world scenarios and document diversity. To address this gap, we introduce OCRTurk, a Turkish document parsing benchmark covering multiple layout elements and document categories at three difficulty levels. OCRTurk consists of 180 Turkish documents drawn from academic articles, theses, slide decks, and non-academic articles. We evaluate seven OCR models on OCRTurk using element-wise metrics. Across difficulty levels, PaddleOCR achieves the strongest overall results, leading most element-wise metrics except figures and attaining high Normalized Edit Distance scores in easy, medium, and hard subsets. We also observe performance variation by document type. Models perform well on non-academic documents, while slideshows become the most challenging.

==> equation_errors_figure.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/equation_errors_figure.png}
    \caption{An output of a model (bottom) compared with the ground truth (top). In the model output, the conditions are not interpreted and the lower limit of the second summation is interpreted incorrectly. The errors are written in red.}
    \label{fig:equation_errors_figure}
\end{figure*}

==> main <==
% Use this file for citations not found in the ACL Anthology (contained in "anthology.bib").


@misc{Yang2024,
    author  = {Z. Yang and J. Tang and Z. Li and P. Wang and J. Wan and H. Zhong and X. Liu and M. Yang and P. Wang and Y. Liu and L. Jin and X. Bai and S. Bai and J. Lin},
    title   = {CC-OCR: A Comprehensive and Challenging {OCR} Benchmark for Evaluating Large Multimodal Models in Literacy},
    volume  = {arXiv:2412.02210},
    year    = {2024},
    url     = {https://arxiv.org/abs/2412.02210},
}
@misc{yilmaz-etal-2025-turkish-ocr-benchmark,
    author  = {Y. Yılmaz and E. G. Hanoğlu and A. G. Özkan and K. Öztoprak},
    title   = {Benchmarking {OCR} and Vision{-}Language Models for {Turkish} Text Recognition: A Comprehensive Evaluation Using Synthetic Data},
    year    = {2025},
    url     = {https://doi.org/10.21203/rs.3.rs-7797886/v1},
}
@article{TurkishOCRSurvey,
  author={G. Öztürk, M. and Ö. Sahin, Durmus and Kiliç, Erdal},
  journal={IEEE Access}, 
  title={{Turkish} Optical Character Recognition Under the Lens: A Systematic Review of Language-Specific Challenges, Dataset Scarcity, and Open-Source Limitations}, 
  year={2025},
  volume={13},
  number={},
  pages={168977-168997},
  keywords={Optical character recognition;Text recognition;Systematic literature review;Surveys;Convolutional neural networks;Accuracy;Systematics;Measurement;Linguistics;Focusing;Classification;deep learning;machine learning;optical character recognition;OCR applications;{Turkish} OCR},
  doi={10.1109/ACCESS.2025.3614147}}

@misc{poznanski-etal-olmocr,
    author  = {J. Poznanski and A. Rangapur and J. Borchardt and J. Dunkelberger and R. Huff and D. Lin and C. Wilhelm and K. Lo and L. Soldaini},
    title   = {olmOCR: Unlocking Trillions of Tokens in {PDFs} with Vision{-}Language Models},
    volume  = {arXiv:2502.18443},
    year    = {2025},
    url     = {https://arxiv.org/abs/2502.18443},

}

@misc{subramani-etal-2021-ocr-survey,
    author  = {N. Subramani and A. Matton and M. Greaves and A. Lam},
    title   = {A Survey of Deep Learning Approaches for {OCR} and Document Understanding},
    volume  = {arXiv:2011.13534},
    year    = {2021},
    url     = {https://arxiv.org/abs/2011.13534},
}

@misc{ouyang-etal-2024-omnidocbench,
    author  = {L. Ouyang and Y. Qu and H. Zhou and J. Zhu and R. Zhang and Q. Lin and B. Wang and Z. Zhao and M. Jiang and X. Zhao and J. Shi and F. Wu and P. Chu and M. Liu and Z. Li and C. Xu and B. Zhang and B. Shi and Z. Tu and C. He},
    title   = {OmniDocBench: Benchmarking Diverse {PDF} Document Parsing with Comprehensive Annotations},
    volume  = {arXiv:2412.07626},
    year    = {2024},
    url     = {https://arxiv.org/abs/2412.07626},
}
@misc{fu-etal-2024-ocrbench-v2,
    author  = {L. Fu and B. Yang and Z. Kuang and J. Song and Y. Li and L. Zhu and Q. Luo and X. Wang and H. Lu and M. Huang and Z. Li and G. Tang and B. Shan and C. Lin and Q. Liu and B. Wu and H. Feng and H. Liu and C. Huang and J. Tang},
    title   = {OCRBench v2: An Improved Benchmark for Evaluating Large Multimodal Models on Visual Text Localization and Reasoning},
    volume  = {arXiv:2501.00321},
    year    = {2024},
    url     = {https://arxiv.org/abs/2501.00321},
}

@misc{du-etal-2025-docptbench,
    author = {Y. Du and P. Chen and X. Ying and Z. Chen},
    title  = {DoCPTBench: Benchmarking End{-}to{-}End Photographed Document Parsing and Translation},
    volume = {arXiv:2511.18434},
    year   = {2025},
    url    = {https://arxiv.org/abs/2511.18434},
}
@misc{yang-etal-2024-cc-ocr,
    author = {Z. Yang and J. Tang and Z. Li and P. Wang and J. Wan and H. Zhong and X. Liu and M. Yang and P. Wang and S. Bai and L. Jin and J. Lin},
    title  = {CC{-}OCR: a Comprehensive and Challenging {OCR} Benchmark for Evaluating Large Multimodal Models in Literacy},
    volume = {arXiv:2412.02210},
    year   = {2024},
    url    = {https://arxiv.org/abs/2412.02210},
}
@misc{kizilirmak-2022-offline-handwriting,
    author = {F. Kizilirmak},
    title  = {Offline Handwriting Recognition Using Deep Learning with Emphasis on Data Augmentation Effects},
    year   = {2022},
    url    = {https://research.sabanciuniv.edu/id/eprint/47179/1/10483904.pdf},
    note   = {Master's thesis, Sabancı University}
}
@article{kuncan-etal-2020-turkish-handwriting,
    author = {M. Kuncan and E. Vardar and K. Kaplan and H. M. Ertun\c{c}},
    title  = {{Turkish} Handwriting Recognition System Using Multi{-}Layer Perceptron},
    year   = {2020},
    url    = {https://doi.org/10.21595/jmai.2020.21502},
    journal   = {Journal of Mechatronics and Artificial Intelligence in Engineering}
}
@article{al-zubaidi-etal-2019-two-dimensional-ocr,
    author  = {E. A. Al-Zubaidi and M. M. Mijwil and A. Sh. Alsaadi},
    title   = {Two{-}Dimensional Optical Character Recognition of Mouse Drawn in {Turkish} Capital Letters Using Multi{-}Layer Perceptron Classification},
    journal = {Journal of Southwest Jiaotong University},
    volume  = {54},
    number  = {4},
    year    = {2019},
    url     = {https://doi.org/10.35741/issn.0258-2724.54.4.4}
}
@misc{sevik-2019-derin-ogrenme,
    author = {A. {\c{S}}evik},
    title  = {Derin {\"O}{\u{g}}renme ile {T{\"u}rk{\c{c}}e} Font ve Karakter Tan{\i}ma},
    year   = {2019},
    url    = {https://acikerisim.duzce.edu.tr/items/ab3e1527-dbed-4fe4-8ca7-18d1917c2f7d},
    note   = {Master's thesis, D{\"u}zce University}
}
@article{bartos-etal-2020-the-dataset,
    author  = {G. E. Bartos and Y. Ho\c{s}can and A. Kauer and \'E. Hajnal},
    title   = {A Multilingual Handwritten Character Dataset: T{-}H{-}E Dataset},
    journal = {Acta Polytechnica Hungarica},
    volume  = {17},
    number  = {9},
    pages   = {141--160},
    year    = {2020},
    url     = {https://doi.org/10.12700/aph.17.9.2020.9.8}
}
@inproceedings{zeer2024cosmos,
  title={Cosmos-LLaVA: Chatting with the Visual},
  author={Zeer, Ahmed and Dogan, Eren and Erdem, Yusuf and {\.I}nce, Elif and Shbib, Osama and Uzun, M. Egemen and Uz, Atahan and Yuce, M. Kaan and Kesgin, H. Toprak and Amasyali, M. Fatih},
  booktitle={2024 8th International Artificial Intelligence and Data Processing Symposium (IDAP)},
  pages={1--7},
  year={2024},
  organization={IEEE}
}
@misc{toraman2026turkbenchbenchmarkevaluatingturkish,
    title={TurkBench: A Benchmark for Evaluating {Turkish} Large Language Models},
    author={Toraman, Çağrı and Sever, Ahmet Kaan and Cengiz, Ayşe Aysu and Arslan, Elif Ecem and Sevinç, Görkem and Birdal, Mete Mert and Güldemir, Yusuf Faruk and Kanburoğlu, Ali Buğra and Felekoğlu, Sezen and Gürlek, Osman and Kantar, Sarp and Kütük, Birsen Şahin and Tufan, Büşra and Genç, Elif and Coşkun, Serkan and Demir, Gupse Ekin and Arayıcı, Muhammed Emin and Dursun, Olgun and Gungor, Onur and Üsküdarlı, Susan and Topraksoy, Abdullah and Darıcı, Esra},
    year={2026},
    eprint={2601.07020},
    archivePrefix={arXiv},
    primaryClass={cs.CL},
    url={https://arxiv.org/abs/2601.07020}
}
@book{lin-etal-2014-microsoft-coco,
    author    = {T.-Y. Lin and M. Maire and S. Belongie and others},
    title     = {Microsoft {COCO}: Common Objects in Context},
    booktitle = {Computer Vision -- {ECCV} 2014},
    pages     = {740--755},
    publisher = {Springer International Publishing},
    year      = {2014},
    url       = {https://doi.org/10.1007/978-3-319-10602-1_48}
}
@misc{belval-textrecognitiondatagenerator,
    author       = {E. Belval},
    title        = {TextRecognitionDataGenerator Repository},
    howpublished = {\url{https://github.com/Belval/TextRecognitionDataGenerator}},

}

@misc{wickrema2025benchmarkingimagesimilaritymetrics,
      title={Benchmarking Image Similarity Metrics for Novel View Synthesis Applications}, 
      author={Wickrema, C. and Leary, S. and Sarkar, S. and Giglio, M. and Bianchi, E. and Mace, E. and Twardowski, M.},
      year={2025},
      eprint={2506.12563},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2506.12563} 
}

@misc{fu2023dreamsimlearningnewdimensions,
      title={DreamSim: Learning New Dimensions of Human Visual Similarity using Synthetic Data}, 
      author={Fu, S. and Tamir, N. and Sundaram, S. and Chai, L. and Zhang, R. and Dekel, T. and Isola, P.},
      year={2023},
      eprint={2306.09344},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2306.09344}
}
@article{hakkani2002statistical,
  title={Statistical morphological disambiguation for agglutinative languages},
  author={Hakkani-Tür, Dilek Z. and Oflazer, Kemal and Tür, Gökhan},
  journal={Computers and the Humanities},
  volume={36},
  number={4},
  pages={381--410},
  year={2002},
  publisher={Springer}
}

@article{oflazer2014turkish,
  title={{Turkish} and its challenges for language processing},
  author={Oflazer, Kemal},
  journal={Language resources and evaluation},
  volume={48},
  number={4},
  pages={639--653},
  year={2014},
  publisher={Springer}
}
@misc{memon2020handwrittenopticalcharacterrecognition,
      title={Handwritten Optical Character Recognition (OCR): A Comprehensive Systematic Literature Review (SLR)}, 
      author={J. Memon and M. Sami and R. A. Khan},
      year={2020},
      eprint={2001.00139},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2001.00139}
}
@inproceedings{Huang_2019,
   title={ICDAR2019 Competition on Scanned Receipt OCR and Information Extraction},
   url={http://dx.doi.org/10.1109/ICDAR.2019.00244},
   DOI={10.1109/icdar.2019.00244},
   booktitle={2019 International Conference on Document Analysis and Recognition (ICDAR)},
   publisher={IEEE},
   author={Huang, Zheng and Chen, Kai and He, Jianhua and Bai, Xiang and Karatzas, Dimosthenis and Lu, Shijian and Jawahar, C. V.},
   year={2019},
   month=sep }
@misc{park2019cord,
  title={CORD: A Consolidated Receipt Dataset for Post-OCR Parsing},
  author={Park, Seunghyun and Shin, Seung and Lee, Bado and Lee, Junyeop and Surh, Jaeheung and Seo, Minjoon and Lee, Hwalsuk},
  booktitle={Document Intelligence Workshop at Neural Information Processing Systems},
  year={2019}
}
@inproceedings{Munjal_2021,
   title={STRIDE: Scene Text Recognition In-Device},
   url={http://dx.doi.org/10.1109/IJCNN52387.2021.9534319},
   DOI={10.1109/ijcnn52387.2021.9534319},
   booktitle={2021 International Joint Conference on Neural Networks (IJCNN)},
   publisher={IEEE},
   author={Munjal, Rachit S. and Prabhu, Arun D. and Arora, Nikhil and Moharana, Sukumar and Ramena, Gopi},
   year={2021},
   month=jul, pages={1–8} }
@inbook{Lunia_2023,
   title={IndicSTR12: A Dataset for Indic Scene Text Recognition},
   ISBN={9783031414985},
   ISSN={1611-3349},
   url={http://dx.doi.org/10.1007/978-3-031-41498-5_17},
   DOI={10.1007/978-3-031-41498-5_17},
   booktitle={Document Analysis and Recognition – ICDAR 2023 Workshops},
   publisher={Springer Nature Switzerland},
   author={Lunia, Harsh and Mondal, Ajoy and Jawahar, C. V.},
   year={2023},
   pages={233–250} }
@misc{heakl2025kitabbenchcomprehensivemultidomainbenchmark,
      title={KITAB-Bench: A Comprehensive Multi-Domain Benchmark for {Arabic} OCR and Document Understanding}, 
      author={Heakl, A. and Sohail, A. and Ranjan, M. and Hossam, R. and Ahmad, G. Shazan and El-Geish, Mohamed and Maher, Omar and Shen, Zhiqiang and Khan, Fahad and Khan, Salman},
      year={2025},
      eprint={2502.14949},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2502.14949}
}
@inproceedings{Anand_2023, 
   series={MM '23},
   title={{TC-OCR}: {TableCraft} {OCR} for Efficient Detection \& Recognition of Table Structure \& Content},
   url={http://dx.doi.org/10.1145/3606040.3617444},
   DOI={10.1145/3606040.3617444},
   booktitle={Proceedings of the 1st International Workshop on Deep Multimodal Learning for Information Retrieval},
   publisher={ACM},
   author={Anand, Avinash and Jaiswal, Raj and Bhuyan, Pijush and Gupta, Mohit and Bangar, Siddhesh and Imam, Md. Modassir and Shah, Rajiv Ratn and Satoh, Shin'ichi},
   year={2023},
   month=oct, 
   pages={11--18},
   collection={MM '23} 
}
@misc{patel2025designimplementationocrpoweredpipeline,
      title={Design and Implementation of an OCR-Powered Pipeline for Table Extraction from Invoices}, 
      author={Parshva Dhilankumar Patel},
      year={2025},
      eprint={2507.07029},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2507.07029}, 
}
@inproceedings{umutlu-etal-2025-evaluating,
    title = "Evaluating the Quality of Benchmark Datasets for Low-Resource Languages: A Case Study on {T}urkish",
    author = "Umutlu, Elif Ecem  and
      Cengiz, Ayse Aysu  and
      Sever, Ahmet Kaan  and
      Erdem, Seyma  and
      Aytan, Burak  and
      Tufan, Busra  and
      Topraksoy, Abdullah  and
      Dar{\i}c{\i}, Esra  and
      Toraman, Cagri",
    editor = "Arviv, Ofir  and
      Clinciu, Miruna  and
      Dhole, Kaustubh  and
      Dror, Rotem  and
      Gehrmann, Sebastian  and
      Habba, Eliya  and
      Itzhak, Itay  and
      Mille, Simon  and
      Perlitz, Yotam  and
      Santus, Enrico  and
      Sedoc, Jo{\~a}o  and
      Shmueli Scheuer, Michal  and
      Stanovsky, Gabriel  and
      Tafjord, Oyvind",
    booktitle = "Proceedings of the Fourth Workshop on Generation, Evaluation and Metrics (GEM{\texttwosuperior})",
    month = jul,
    year = "2025",
    address = "Vienna, Austria and virtual meeting",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2025.gem-1.41/",
    pages = "471--487",
    ISBN = "979-8-89176-261-9",
}
@misc{pallavi2020conglomeratemultipleocrtable,
      title={A Conglomerate of Multiple OCR Table Detection and Extraction}, 
      author={Smita Pallavi and Raj Ratn Pranesh and Sumit Kumar},
      year={2020},
      eprint={2010.08591},
      archivePrefix={arXiv},
      primaryClass={cs.IR},
      url={https://arxiv.org/abs/2010.08591}, 
}
@misc{zhong2025doctronformulageneralizedformularecognition,
      title={DocTron-Formula: Generalized Formula Recognition in Complex and Structured Scenarios}, 
      author={Yufeng Zhong and Zhixiong Zeng and Lei Chen and Longrong Yang and Liming Zheng and Jing Huang and Siqi Yang and Lin Ma},
      year={2025},
      eprint={2508.00311},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2508.00311}, 
}
@article{Sayallar2023,
title = {An OCR Engine for Printed Receipt Images using Deep Learning Techniques},
journal = {International Journal of Advanced Computer Science and Applications},
doi = {10.14569/IJACSA.2023.0140295},
url = {http://dx.doi.org/10.14569/IJACSA.2023.0140295},
year = {2023},
publisher = {The Science and Information Organization},
volume = {14},
number = {2},
author = {Cagri Sayallar and Ahmet Sayar and Nurcan Babalik}
}
@article{b20eb0cbcfa7411d83518db7a94b879a,
title = "Information Extraction from Text Intensive and Visually Rich Banking Documents",
abstract = "Document types, where visual and textual information plays an important role in their analysis and understanding, pose a new and attractive area for information extraction research. Although cheques, invoices, and receipts have been studied in some previous multi-modal studies, banking documents present an unexplored area due to the naturalness of the text they possess in addition to their visual richness. This article presents the first study which uses visual and textual information for deep-learning based information extraction on text-intensive and visually rich scanned documents which are, in this instance, unstructured banking documents, or more precisely, money transfer orders. The impact of using different neural word representations (i.e., FastText, ELMo, and BERT) on IE subtasks (namely, named entity recognition and relation extraction stages), positional features of words on document images and auxiliary learning with some other tasks are investigated. The article proposes a new relation extraction algorithm based on graph factorization to solve the complex relation extraction problem where the relations within documents are n-ary, nested, document-level, and previously indeterminate in quantity. Our experiments revealed that the use of deep learning algorithms yielded around 10 percentage points improvement on the IE sub-tasks. The inclusion of word positional features yielded around 3 percentage points of improvement in some specific information fields. Similarly, our auxiliary learning experiments yielded around 2 percentage points of improvement on some information fields associated with the specific transaction type detected by our auxiliary task. The integration of the information extraction system into a real banking environment reduced cycle times substantially. When compared to the manual workflow, document processing pipeline shortened book-to-book money transfers to 10 minutes (from 29 min.) and electronic fund transfers (EFT) to 17 minutes (from 41 min.) respectively.",
keywords = "Banking Documents, Deep Learning, Information Extraction, NLP in Finance, Named Entity Recognition, Relation Extraction, Text Intensive Documents, Visually Rich Documents",
author = "Berke Oral and Erdem Emekligil and Se{\c c}il Arslan and G{\"u}l{\c s}en Eryiǧit",
year = "2020",
month = nov,
doi = "10.1016/j.ipm.2020.102361",
language = "English",
volume = "57",
journal = "Information Processing and Management",
issn = "0306-4573",
publisher = "Elsevier Ltd",
number = "6",
}


==> metric_comparison_wrt_category.tex <==
\begin{figure*}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=1.1\textwidth,
            height=8.5cm,
            ybar=0.4pt,
            bar width=11pt,h
            ylabel={Score},
            xlabel={Category},
            symbolic x coords={Academic, NonAcademic, Theses, Slideshow}, 
            xtick=data,
            xticklabels={Academic Docs., Non-academic Docs., Theses, Slideshow}, 
            ymin=0.7, ymax=1,        
            ytick={0.6, 0.7, 0.8, 0.9, 1.0},
            enlarge x limits=0.2,
            legend style={
                at={(0.5,-0.25)}, 
                anchor=north, 
                legend columns=4,
                font=\footnotesize,
                draw=none,
                /tikz/every even column/.append style={column sep=5pt}
            },
            nodes near coords,
            every node near coord/.append style={
                font=\tiny, 
                rotate=90, 
                anchor=west,
                color=black,
                /pgf/number format/fixed,
                /pgf/number format/precision=2
            },
            ymajorgrids=true,
            grid style={dashed,gray!30},
            axis line style={draw=gray!60}
        ]
            \addplot[fill=blue7, draw=blue7!70!black] table [x=Category, y=deepseek, col sep=comma] {triplets_wrt_category.csv};
            \addplot[fill=blue6, draw=blue6!70!black] table [x=Category, y=docling,  col sep=comma] {triplets_wrt_category.csv};
            \addplot[fill=blue5, draw=blue5!70!black] table [x=Category, y=huanyan,  col sep=comma] {triplets_wrt_category.csv};
            \addplot[fill=blue4, draw=blue4!70!black] table [x=Category, y=nanonets, col sep=comma] {triplets_wrt_category.csv};
            \addplot[fill=blue3, draw=blue3!70!black] table [x=Category, y=nvidia,   col sep=comma] {triplets_wrt_category.csv};
            \addplot[fill=blue2, draw=blue2!70!black] table [x=Category, y=olmocr,   col sep=comma] {triplets_wrt_category.csv};
            \addplot[fill=blue1, draw=blue1!70!black] table [x=Category, y=paddle,   col sep=comma] {triplets_wrt_category.csv};
            
            \draw [red, thick, dashed] ([xshift=-45pt]axis cs:Academic, 0.886) -- ([xshift=45pt]axis cs:Academic, 0.886)
            node[right, font=\tiny] {$0.89$};
            
            \draw [red, thick, dashed] ([xshift=-45pt]axis cs:NonAcademic, 0.937) -- ([xshift=45pt]axis cs:NonAcademic, 0.937)
            node[right, font=\tiny] {$0.94$};
            
            \draw [red, thick, dashed] ([xshift=-45pt]axis cs:Theses, 0.906) -- ([xshift=45pt]axis cs:Theses, 0.906)
            node[right, font=\tiny] {$0.91$};

            \draw [red, thick, dashed] ([xshift=-45pt]axis cs:Slideshow, 0.858) -- ([xshift=45pt]axis cs:Slideshow, 0.858)
            node[right, font=\tiny] {$0.86$};

            \legend{DeepSeekOCR, Docling, HuanyanOCR, NanonetsOCR2, Nvidia Nemotron v1.1, OlmOCR2, PaddleOCR}
günc        \end{axis}
    \end{tikzpicture}
    \caption{Comparison of the models DeepSeekOCR, Docling, PaddleOCR, HuanyanOCR, NanonetsOCR2, Nvidia Nemotron v1.1, and OlmOCR under the categories academic documents, non-academic documents, theses, and slideshows. The scores are the averages of the NED metric scores for raw texts, tables, and equations of the data within the same difficulty. The NED scores are subtracted from 1 ($\text{Score} = 1 - \text{NED}$) for better comparison. The average score of the models within each category is given as the dashed red line.} 
    \label{fig:metric_comparison_wrt_category}
\end{figure*}

==> metric_comparison_wrt_difficulty.tex <==
\begin{figure*}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=\textwidth,
            height=8.5cm,
            ybar=0.4pt,
            bar width=11pt,
            ylabel={Score},
            xlabel={Difficulty Level},
            symbolic x coords={easy, medium, hard},
            xtick=data,
            xticklabels={Easy, Medium, Hard}, 
            ymin=0.6, ymax=1.05,
            ytick={0.6, 0.7, 0.8, 0.9, 1.0},
            enlarge x limits=0.25,      
            legend style={
                at={(0.5,-0.25)}, 
                anchor=north, 
                legend columns=4,
                font=\footnotesize,
                draw=none,
                /tikz/every even column/.append style={column sep=5pt}
            },
            nodes near coords,
            every node near coord/.append style={
                font=\tiny, 
                rotate=90, 
                anchor=west,
                color=black,
                /pgf/number format/fixed,
                /pgf/number format/precision=2
            },
            ymajorgrids=true,
            grid style={dashed,gray!30},
            axis line style={draw=gray!60}
        ]
            \addplot[fill=blue7, draw=blue7!70!black] table [x=Difficulty, y=deepseek, col sep=comma] {triplets_wrt_difficulty.csv};
            \addplot[fill=blue6, draw=blue6!70!black] table [x=Difficulty, y=docling,  col sep=comma] {triplets_wrt_difficulty.csv};
            \addplot[fill=blue5, draw=blue5!70!black] table [x=Difficulty, y=huanyan,  col sep=comma] {triplets_wrt_difficulty.csv};
            \addplot[fill=blue4, draw=blue4!70!black] table [x=Difficulty, y=nanonets, col sep=comma] {triplets_wrt_difficulty.csv};
            \addplot[fill=blue3, draw=blue3!70!black] table [x=Difficulty, y=nvidia,   col sep=comma] {triplets_wrt_difficulty.csv};
            \addplot[fill=blue2, draw=blue2!70!black] table [x=Difficulty, y=olmocr,   col sep=comma] {triplets_wrt_difficulty.csv};
            \addplot[fill=blue1, draw=blue1!70!black] table [x=Difficulty, y=paddle,   col sep=comma] {triplets_wrt_difficulty.csv};
            
            \draw [red, thick, dashed] ([xshift=-40pt]axis cs:easy, 0.98) -- ([xshift=40pt]axis cs:easy, 0.98)
            node[right, font=\tiny] {$0.98$};
            \draw [red, thick, dashed] ([xshift=-40pt]axis cs:medium, 0.91) -- ([xshift=40pt]axis cs:medium, 0.91)
            node[right, font=\tiny] {$0.91$};
            \draw [red, thick, dashed] ([xshift=-40pt]axis cs:hard, 0.80) -- ([xshift=40pt]axis cs:hard, 0.80)
            node[right, font=\tiny] {$0.81$};

            \legend{DeepSeekOCR, Docling, HuanyanOCR, NanonetsOCR2, Nvidia Nemotron v1.1, OlmOCR2, PaddleOCR}
        \end{axis}
    \end{tikzpicture}
    \caption{Comparison of the models DeepSeekOCR, Docling, PaddleOCR, HuanyanOCR, NanonetsOCR2, Nvidia Nemotron v1.1, and OlmOCR under easy, medium, and hard data. The scores are the averages of the NED metric scores for raw texts, tables, and equations of the data within the same difficulty. The NED scores are subtracted from 1 ($\text{Score} = 1 - \text{NED}$) for better comparison. The average score of the models within each difficulty level is given as the dashed red line.} 
    \label{fig:metric_comparison_wrt_difficulty}
\end{figure*}
